Distributed Task Allocation in Homogeneous Swarms Using Language Measure Theory

In this paper, we present algorithms for synthesizing controllers to distribute a group (possibly swarms) of homogeneous robots (agents) over heterogeneous tasks which are operated in parallel. We present algorithms as well as analysis for global and local-feedback-based controller for the swarms. Using ergodicity property of irreducible Markov chains, we design a controller for global swarm control. Furthermore, to provide some degree of autonomy to the agents, we augment this global controller by a local feedback-based controller using Language measure theory. We provide analysis of the proposed algorithms to show their correctness. Numerical experiments are shown to illustrate the performance of the proposed algorithms.

==> background.tex <==
\section{Background}\label{sec:background}
In this section, we provide some preliminary concepts and notations that facilitate understanding of the concepts presented in the sequel. We denote the cardinality of any set $\Phi$  by $|\Phi |$.
\begin{definition}\label{def:MC}
 A finite-state homogeneous Markov chain is a triple $G=(Q, \textbf{P} ,\mathbf{p}^{[0]})$, where Q is the set of states with $|Q|=M$ $\in$ $\natural$, $\textbf{P}$ is the $M \times M$ 
stationary probability matrix such that $\forall$ $i,j$ $\in$ $\{1,\dots ,M\},$ $\textbf{P}_{ij}\geqq 0$ with $\sum\limits_{j=1}^{M} {\textbf{P}_{ij}}=1$, and $\mathbf{p}^{[0]} \in [0,1]^{|Q|}$, $\sum\limits_{i=1}^{M} {\mathbf{p}^{[0]}_i} =1$, is the initial distribution over the states.
\end{definition}
\begin{definition}\label{def:HMC}
A finite-state homogeneous Markov chain $G=(Q, \textbf{P} ,\mathbf{p}^{[0]})$, with $|Q|=M,\, M\geq 2$, is called irreducible if, for any $(i,j),\,1\leq i,j \leq M$, 
there exists a finite positive integer $k(i,j)$ such that the $ij$th element of the $k$th power of $\textbf{P}$ is strictly positive, i.e., $\textbf{P}^k_{ij}>0$. In this case, the stochastic transition 
matrix $\textbf{P}$ is also an irreducible matrix~\cite{BR97}. 
\end{definition}

The transition matrix of a finite Markov chain is always a stochastic matrix~\cite{BR97}. Any stochastic transition matrix $\textbf{K}$ has at least one unity eigenvalue, 
and all the eigenvalues of $\textbf{K}$ are located within or on the unit disc. For any $M\times M$ irreducible stochastic matrix $\textbf{K}$ with $M >1$, the diagonal terms are strictly less than unity, 
i.e., $\textbf{K}_{ii}<1\, \forall i$. Upon unity sum normalization, the left eigenvector $P=[P_1, P_2,\dots, P_M]$ corresponding to the unique unity eigenvalue of
$\textbf{K}$ is called the stationary probability vector, where $\sum\limits_i{{P}_i}=1$, and ${P}_j>0 \,\quad \forall $ $j \in \{1,2,\dots,M\}$~\cite{BR97} such that $P\textbf{K}=P$. We use this property of irreducible stochastic matrices in the design of the controller for the swarm.% which we will discuss in detail in later sections.


Next we present a brief review of language measure theory~ \cite{CR07, JLWR15} which is later used to synthesize the distributed architecture for the problem discussed in this paper.
\subsection{Review of Language Measure of a Probabilistic Finite State Automata}
This section summarizes the concept of signed real measure of probabilistic finite state automata (PFSA) and its role for optimal control of PFSA.
While the theories of language measure and the associated optimal control are developed in~\cite{R05}\cite{CR07}, this section introduces pertinent definitions and summarizes the essential concepts that are used in the sequel.


\begin{definition}  (PFSA) \label{def:PFSA} A probabilistic finite state automaton (PFSA) over an alphabet $\Sigma$ is a quintuple $$\mathbb{G} \triangleq (Q,\Sigma,\delta,\Pi,\mbox{\boldmath $\chi$}), \ \textrm{where}$$
\begin{itemize}
\item $Q$ is the nonempty finite set of states, i.e., $|Q| \in \mathbb{N}$;
\item $\delta: Q\times \Sigma^\star \rightarrow Q$ is the transition map that satisfies the following conditions: $\forall q\in Q \ \ \forall s \in \Sigma \ \ \forall w \in \Sigma^\star$ \\ $\delta(q,\epsilon) =q$;  and    $\delta(q, ws) = \delta\big(\delta(q,w), s \big )$.
\item $\Pi:Q \times \Sigma^\star \rightarrow [0,1]$ is the morph function of state-specific symbol generation probabilities, which satisfies the following conditions: $\forall q\in Q \ \ \forall s \in \Sigma \ \ \forall w \in \Sigma^\star$ \\ $\Pi(q,s)\geq 0$; \ $\sum_{s \in \Sigma}\Pi(q,s)=1$; and \\ $\Pi(q,\epsilon)=1$; $\Pi(q, ws) = \Pi(q,w) \times \Pi(\delta(q,w),s)$.
\item  $\mbox{\boldmath $\chi$}:Q \rightarrow [-1, 1]^{|Q|}$ is the vector-valued characteristic function that assigns a signed (normalized)
real weight to each state.
\end{itemize}

The $(|Q| \times |Q|)$ state transition probability matrix $\textbf{P}$ is defined as
$$\textbf{P}=[\textbf{P}_{jk}], \ \textrm{where} \ \textbf{P}_{jk}\triangleq \sum_{s \in \Sigma: \ \delta(q_j,s)=q_k} \Pi(q_j,s) \ \forall q_j, q_k \in Q$$
Note: $\textbf{P}$ is a non-negative stochastic matrix~\cite{BR97}. It is also noted that a PFSA induces a Markov chain $\mathbb{M}=(Q,\textbf{P},\textbf{p}^{[0]})$ where $\textbf{p}^{[0]}$ is the one-hot vector representing the initial state of the PFSA.% where $\textbf{P}_{ij}$ is the probability of transition from $q_i$ to $q_j$.\\
\end{definition}

We skip some definition and details for brevity. Interested readers are refered to~\cite{JLWR15} for details about the same. We present definition of language induced by a PFSA before presenting the definition of the real measure for the same.


\begin{definition} (Language) \label{def:Language} Let $(Q,\Sigma,\delta,\Pi,\mbox{\boldmath $\chi$})$ be a PFSA. The language generated by all words, which terminates at a state $q_k \in Q$ after starting from $q_j \in Q$, is defined as
\begin{equation}\label{eq:Language_jk}
L(q_j, q_k) \triangleq \{w \in \Sigma^*: \ \delta^\star(q_j,w)=q_k\}
\end{equation}
The language generated by all words, which may terminate at any state $q \in Q$ after starting from $q_j \in Q$, is defined as
\begin{equation}\label{eq:Language}
L(q_j) \triangleq \bigcup_{q \in Q}L(q_j, q)
\end{equation}
\end{definition}

Given a PFSA $(Q,\Sigma,\delta, \Pi,\mbox{\boldmath $\chi$})$, the following facts are considered before the notion of a measure is introduced on the language $L$ (see  Definition~\ref{def:Language}).
\begin{itemize}
\item The language $L$ is an at most countable (i.e., finite or countably infinite) set because $L \subseteq \Sigma^\star$. Therefore, the power set $2^L$ is either finite or uncountable; if uncountable, the cardinality of $2^L$ is the same as that of $\mathbb{R}$ or that of the standard Borel algebra $\mathcal{B}(\mathbb{R})$~\cite{royden1988real}.
\item A measurable space $(L,\Sigma^\omega2^L)$ can be constructed where every singleton set of a semi-infinite string of symbols, whose suffix is a word in $L$, is a measurable set. For brevity, the $\sigma$-algebra $\Sigma^\omega2^L$ is denoted as $2^L$, because every word $w \in L$ is prefixed by a semi-infinite string of symbols. That is, $w$ represents $xw$ and $\{w\} \in 2^L$ implies $\{xw\}\in\Sigma^\omega2^L$, where $x \in \Sigma^\omega$ is arbitrary.
\end{itemize}

\begin{definition}(Language Measure)\label{def:LanguageMeasure} Let $L(q_j,q_k)$ and $L(q_j)$ be languages on a PFSA $(Q,\Sigma,\delta,\pi,\mbox{\boldmath $\chi$})$ and let $\theta \in (0,1)$ be a parameter. A signed real measure $\mu^{jk}_\theta: \ 2^{L(q_j,q_k)}\rightarrow \mathbb{R}$ (that satisfies the requisite axioms of measure ~\cite{royden1988real}) is defined as
\begin{equation}\label{eq:LanguageMeasure_jk}
\mu^{jk}_{\theta}(L(q_j,q_k))\triangleq \sum_{w\in L(q_j,q_k)}\theta(1-\theta)^{|w|}\pi(q_j,w)\mbox{\boldmath $\chi$}(q_k)
\end{equation}
The measure of the language $L(q_j)$ is defined as
\begin{equation}\label{eq:LanguageMeasure}
\nu^j_{\theta}(L(q_j))\triangleq \sum_{q_k \in Q} \ \mu^{jk}_{\theta}(L(q_j,q_k))
\end{equation}
\end{definition}

Following Definition~\ref{def:LanguageMeasure} the set of language measures  for a PFSA is interpreted as a real-valued vector of dimension $|Q|$ and is denoted as $\mbox{\boldmath $\nu$}_\theta$ whose $j^{th}$ component is $\nu^j_{\theta}\in \mathbb{R}$ corresponding to the state $q_j \in Q$. Following Theorem 1 in~\cite{R05}, the language measure of the PFSA $(Q,\Sigma,\delta,\pi,\mbox{\boldmath $\chi$})$ in Eq.~(\ref{def:LanguageMeasure}) is expressed vectorially as
\begin{equation} \label{eq:VectorMeasure}
 \mbox{\boldmath $\nu$}_\theta = \theta [\mathbb{I}-(1-\theta) \textbf{P}]^{-1} \mbox{\boldmath $\chi$}
\end{equation}
where $\textbf{P}$ is the state transition matrix (see Definition~\ref{def:PFSA}) and the inverse on the right side exists for all $\theta \in (0,1)$.
Furthermore, as \ $\theta \rightarrow 0^+$, the matrix
$\theta [\mathbb{I}-(1-\theta) \textbf{P}]^{-1}$ converges to the Cesaro matrix $\mbox{\boldmath $\mathcal{P}$} \triangleq \lim_{k \rightarrow \infty} \frac{1}{k}\sum\limits_{j=0}^{k-1} \textbf{P}^j$.
Then, the limiting measure vector $\mbox{\boldmath $\nu$}_0$ is obtained as~\cite{CR07}
\begin{equation}\label{eq:VectorMeasureZero}
\mbox{\boldmath $\nu$}_0 \triangleq \lim_{\theta \rightarrow 0^+} \mbox{\boldmath $\nu$}_\theta = \lim_{\theta \rightarrow 0^+} \theta [\mathbb{I}-(1-\theta) \textbf{P}]^{-1} \mbox{\boldmath $\chi$}= \mbox{\boldmath $\mathcal{P}$} \ \mbox{\boldmath $\mbox{\boldmath $\chi$}$}
\end{equation}
where $\mathbb{I}$ is the $(|Q|\times |Q|)$ identity matrix.

The limiting language measure $\nu_0^j$ sums up to the limiting real measure of each string starting from state $q_j$, given the weighting function, $\mbox{\boldmath $\chi$}$. Thus $\nu_0^j$ captures the goodness of $q_j$ based on not only its own characteristic weight but also on how good are strings that will be generated from $q_j$ in the future. And thus the limiting language measure provides a quantitative comparison of the states of the PFSA (and thus the Markov chain). A state with higher and positive measure denotes a \textit{good} state when compared to a state with lower measure. For readers familiar with dynamic programming for infinite horizon, the parameter $(1-\theta)$ is analogous to the discount factor used in value iterations~\cite{bertsekas1995dynamic}. As a result, the values closer to $1$ for $(1-\theta)$ work well for computing the infinite horizon language measure. Interested readers to refered to earlier publications~\cite{CR07} for discussion on selection of the parameter $\theta$. 
%\textbf{{Definition $5$ (Controlled descendant):}} Let the Markov chain $G=(Q,\Pi,P^0)$ be derived from a finite-state Markov chain $\tilde{G}=(Q,\tilde{\Pi},P^0)$. Then, $G$ is defined to be a controlled descendant of $\tilde{G}$ if the following condition is satisfied:
%\begin{equation}
%^ \forall i\neq j, \tilde{\Pi}_{ij}=0 \Rightarrow \Pi_{ij}=0.
%\end{equation}
%A descendant $G$ is obtained by probabilistic enabling or disabling to one or more transitions of the Markov chain $\tilde{G}$.
